Wireless Connectivity and Localization for Advanced Air Mobility Services

By serving as an analog to traffic signal lights, communication signaling for drone to drone communications holds the key to the success of advanced air mobility (AAM) in both urban and rural settings. Deployment of AAM applications such as air taxis and air ambulances, especially at large-scale, requires a reliable channel for a point-to-point and broadcast communication between two or more aircraft. Achieving such high reliability, in a highly mobile environment, requires communication systems designed for agility and efficiency. This paper presents the foundations for establishing and maintaining a reliable communication channel among multiple aircraft in unique AAM settings. Subsequently, it presents concepts and results on wireless coverage and mobility for AAM services using cellular networks as a ground network infrastructure. Finally, we analyze the wireless localization performance at 3D AAM corridors when cellular networks are utilized, considering different corridor heights and base station densities. We highlight future research directions and open problems to improve wireless coverage and localization throughout the manuscript.

==> D2DComms.tex <==
\section{Drone-to-Drone Communications or Air Corridors}
- Links to AG systems
-PHY \& MAC considerations \& future work

\subsection{A2A Channel Models - David}
\subsection{Technologies: ADS-B, LDACS, Renote ID, etc - David and Kamesh}
